The Klarna Product Page Dataset: Web Element Nomination with Graph Neural Networks and Large Language Models

Web automation holds the potential to revolutionize how users interact with the digital world, offering unparalleled assistance and simplifying tasks via sophisticated computational methods. Central to this evolution is the web element nomination task, which entails identifying unique elements on webpages. Unfortunately, the development of algorithmic designs for web automation is hampered by the scarcity of comprehensive and realistic datasets that reflect the complexity faced by real-world applications on the Web. To address this, we introduce the Klarna Product Page Dataset, a comprehensive and diverse collection of webpages that surpasses existing datasets in richness and variety. The dataset features 51,701 manually labeled product pages from 8,175 e-commerce websites across eight geographic regions, accompanied by a dataset of rendered page screenshots. To initiate research on the Klarna Product Page Dataset, we empirically benchmark a range of Graph Neural Networks (GNNs) on the web element nomination task. We make three important contributions. First, we found that a simple Convolutional GNN (GCN) outperforms complex state-of-the-art nomination methods. Second, we introduce a training refinement procedure that involves identifying a small number of relevant elements from each page using the aforementioned GCN. These elements are then passed to a large language model for the final nomination. This procedure significantly improves the nomination accuracy by 16.8 percentage points on our challenging dataset, without any need for fine-tuning. Finally, in response to another prevalent challenge in this field - the abundance of training methodologies suitable for element nomination - we introduce the Challenge Nomination Training Procedure, a novel training approach that further boosts nomination accuracy.

==> tables/classification-table <==
\begin{small}
    \begin{tabular}{rccccccc}
        \toprule
        & buy button & cart button & product image & name & price & subject node & avg. \\
        \midrule
        \textsc{LSTM-Bi} &
    .91/.95 & \textbf{.92/.95} & \textbf{.89/.94} & .93/.89 & .85/.90 & .96/.91 & .95/.95\\
        \textsc{LSTM-BiE} &
    \textbf{.97/.92} & .95/.89 & .92/.85 & .92/.91 & .90/.86 & \textbf{.96/.96} & .95/.95\\
        \textsc{GCN-GRU} &
    .95/.92 & .93/.86 & .90/.88 & .90/.90 & .89/.85 & .95/.93 & .94/.94\\
        \textsc{FreeDOM} &
    .80/.93 & .45/.88 & .50/.43 & .91/.88 & .86/.88 & .96/.33 & .84/.82\\
        \textsc{FreeDOM-ext} &
    .95/.95 & .92/.88 & .89/.90 & \textbf{.97/.95} & \textbf{.96/.94} & .92/.91 & \textbf{.95/.95} \\
        \textsc{FCN} &
    .96/.91 & .94/.81 & .91/.80 & .89/.91 & .83/.88 & .93/.94 & .93/.93\\
        \textsc{LSTM-TD} &
    .94/.93 & .93/.86 & .90/.83 & .92/.91 & .90/.85 & .94/.90 & .94/.94\\
        \textsc{TE} &
    .91/.94 & .90/.94 & .88/.91 & .92/.90 & .84/.93 & .95/.91 & .95/.95\\
        \textsc{GCN-Mean} &
    .97/.90 & .96/.80 & .94/.85 & .93/.92 & .93/.84 & .97/.91 & .94/.94\\
        \bottomrule
    \end{tabular}
\end{small}



% \begin{footnotesize}
%     \begin{tabular}{rccccccc}
%         \toprule
%         & BuyButton & Cart & Picture & Name & Price & SubjectNode & Avg. \\
%         \midrule
%         \textsc{LSTM-Bi} &
%     .919/.952/.935 & \textbf{.929/.951/.940} & \textbf{.890/.943/.915} & .933/.891/.912 & .854/.908/.880 & .967/.918/.942 & .954/.953/.954\\
%         \textsc{LSTM-BiE} &
%     \textbf{.971/.922/.946} & .957/.894/.924 & .929/.858/.892 & .927/.912/.919 & .900/.865/.882 & \textbf{.962/.965/.963} & .954/.955/.954\\
%         \textsc{DOM-Q-NET} &
%     .959/.927/.943 & .936/.865/.899 & .904/.889/.897 & .907/.907/.907 & .891/.858/.874 & .952/.930/.941 & .947/.948/.947\\
%         \textsc{FreeDOM} &
%     .809/.938/.868 & .450/.887/.596 & .508/.437/.469 & .915/.888/.901 & .869/.882/.875 & .964/.338/.500 & .847/.823/.822\\
%         \textsc{FreeDOM-ext} &
%     .958/.959/.959 & .921/.889/.905 & .890/.900/.895 & \textbf{.977/.953/.965} & \textbf{.965/.941/.953} & .927/.917/.922 & \textbf{.958/.958/.958} \\
%         \textsc{FCN} &
%     .960/.918/.939 & .944/.814/.875 & .910/.801/.852 & .894/.918/.906 & .839/.885/.861 & .933/.944/.938 & .939/.939/.938\\
%         \textsc{GAT} &
%     .720/.884/.794 & .844/.737/.787 & .898/.326/.479 & .821/.837/.829 & .535/.798/.641 & .380/.393/.386 & .812/.799/.796\\
%         \textsc{LSTM-TD} &
%     .944/.931/.936 & .931/.867/.897 & .901/.835/.866 & .920/.913/.916 & .903/.859/.880 & .948/.906/.926 & .944/.944/.944\\
%         \textsc{TE} &
%     .915/.944/.929 & .902/.941/.921 & .888/.917/.902 & .922/.904/.913 & .847/.936/.889 & .954/.918/.936 & .951/.950/.950\\
%         \textsc{PinSage} &
%     .973/.900/.935 & .967/.806/.879 & .945/.858/.899 & .931/.920/.925 & .933/.848/.889 & .979/.910/.943 & .949/.949/.948\\
%         \bottomrule
%     \end{tabular}
% \end{footnotesize}
% 


%  RAW DATA
% BidirectionalLSTM
% -----------------
% .919/.952/.935
% .929/.951/.940
% .890/.943/.915
% .933/.891/.912
% .854/.908/.880
% .967/.918/.942
% .954/.953/.954
% 
% 
% BidirectionalLSTMWithEmbeddings
% -------------------------------
% .971/.922/.946
% .957/.894/.924
% .929/.858/.892
% .927/.912/.919
% .900/.865/.882
% .962/.965/.963
% .954/.955/.954
% 
% 
% DOMQNET
% -------
% .959/.927/.943
% .936/.865/.899
% .904/.889/.897
% .907/.907/.907
% .891/.858/.874
% .952/.930/.941
% .947/.948/.947
% 
% 
% FullyConnected
% --------------
% .960/.918/.939
% .944/.814/.875
% .910/.801/.852
% .894/.918/.906
% .839/.885/.861
% .933/.944/.938
% .939/.939/.938
% 
% 
% GAT
% ---
% .720/.884/.794
% .844/.737/.787
% .898/.326/.479
% .821/.837/.829
% .535/.798/.641
% .380/.393/.386
% .812/.799/.796
% 
% 
% TopDownLSTM
% -----------
% .944/.931/.936
% .931/.867/.897
% .901/.835/.866
% .920/.913/.916
% .903/.859/.880
% .948/.906/.926
% .944/.944/.944
% 
% 
% TransformerEncoder
% ------------------
% .915/.944/.929
% .902/.941/.921
% .888/.917/.902
% .922/.904/.913
% .847/.936/.889
% .954/.918/.936
% .951/.950/.950
% 
% 
% TwoLayerGCN
% -----------
% .973/.900/.935
% .967/.806/.879
% .945/.858/.899
% .931/.920/.925
% .933/.848/.889
% .979/.910/.943
% .949/.949/.948
% 
% 
% FreeDOM (Stage 1)
% -----------------
% .809/.938/.868
% .450/.887/.596
% .508/.437/.469
% .915/.888/.901
% .869/.882/.875
% .964/.338/.500
% .847/.823/.822



==> tables/classification-text-table.tex <==
\begin{small}
    \begin{tabular}{rccccccc}
        \toprule
        & buy button & cart button & product image & name & price & subject node & avg. \\
        \midrule
\textsc{LSTM-BU-T} & .92/.98 & \textbf{.92/.95} & .88/.92 & .97/.94 & .92/.92 & .95/.93 & .96/.96\\
\textsc{GCN-GRU-T} & .95/.97 & .91/.94 & \textbf{.88/.93} & .98/.92 & .91/.92 & .94/.95 & \textbf{.96/.96}\\
\textsc{FreeDOM} & .80/.93 & .45/.88 & .50/.43 & .91/.88 & .86/.88 & .96/.33 & .84/.82\\
\textsc{FreeDOM-ext} & .95/.95 & .92/.88 & .89/.90 & .97/.95 & \textbf{.96/.94} & .92/.91 & .95/.95\\
\textsc{FCN-T} & .95/.96 & .91/.95 & .86/.92 & .97/.96 & .87/.94 & .92/.96 & .95/.95\\
\textsc{LSTM-TD-T} & .93/.97 & .93/.94 & .87/.93 & .97/.93 & .92/.90 & .93/.91 & .95/.95\\
\textsc{TE-T} & .93/.97 & .90/.88 & .89/.89 & .96/.94 & .85/.96 & .96/.93 & .95/.95\\
\textsc{GCN-Mean-T} & \textbf{.98/.96} & .96/.90 & .95/.78 & \textbf{.98/.95} & .95/.89 & \textbf{.98/.94} &
\textbf{.96/.96}\\
        \bottomrule
    \end{tabular}
\end{small}


% RAW DATA
% method,Avg.,addtocart,cart,mainpicture,name,price,subjectnode
% BottomUP-T,0.961/0.960/0.961,0.929/0.980/0.954,0.923/0.953/0.938,0.882/0.925/0.903,0.972/0.947/0.959,0.927/0.921/0.924,0.956/0.938/0.947
% DOMQNET-T,0.962/0.962/0.962,0.950/0.971/0.960,0.916/0.949/0.932,0.884/0.933/0.908,0.983/0.928/0.955,0.910/0.924/0.917,0.946/0.959/0.952
% FreeDOM,0.847/0.823/0.822,0.809/0.938/0.869,0.450/0.887/0.597,0.508/0.436/0.470,0.915/0.888/0.901,0.869/0.882/0.875,0.964/0.338/0.500
% FreeDOM-ext,0.958/0.958/0.958,0.958/0.959/0.959,0.921/0.889/0.905,0.890/0.900/0.895,0.977/0.953/0.965,0.965/0.941/0.953,0.927/0.917/0.922
% FullyConnected-T,0.959/0.957/0.958,0.952/0.968/0.960,0.910/0.959/0.934,0.863/0.925/0.893,0.972/0.960/0.966,0.870/0.941/0.904,0.929/0.960/0.944
% TopDown-T,0.957/0.957/0.957,0.936/0.972/0.954,0.932/0.940/0.936,0.871/0.937/0.903,0.978/0.937/0.957,0.922/0.907/0.915,0.935/0.912/0.924
% TransformerEncoder-T,0.955/0.954/0.954,0.939/0.971/0.955,0.906/0.885/0.895,0.891/0.899/0.895,0.964/0.943/0.953,0.853/0.965/0.905,0.964/0.938/0.951
% TwoLayerGCN-T,0.962/0.962/0.961,0.983/0.960/0.971,0.963/0.902/0.931,0.955/0.787/0.863,0.984/0.950/0.967,0.952/0.893/0.921,0.986/0.943/0.964


==> tables/prediction-table.tex <==
\begin{small}
    \begin{tabular}{rccccccc}
        \toprule
        & buy button & cart button & product image & name & price & subject node & avg. \\
        \midrule
        \textsc{LSTM-Bi} & .720 & .570 & .466 & .693 & .483 & .656 & .598 \\
        \textsc{LSTM-BiE} & .773 & .596 & .503 & .724 & .546 & .702 & .641 \\
        \textsc{GCN-GRU} & .775 &.576 & .400 & .700 & .504 & .462 & .569 \\
        \textsc{FreeDOM} & .379 & .061 & .020 & .645 & .245 & .334 & .281 \\
        \textsc{FreeDOM-ext} & \textbf{.840} & .588 & .343 & \textbf{.835} & \textbf{.728} & .479 & .635 \\
        \textsc{FCN} & .786 & .530 & .320 & .702 & .575 & .433 & .558 \\
        \textsc{LSTM-TD} & .714 & .512 & .424 & .696 & .523 & .584 & .575 \\
        \textsc{TE} & .708 & .468 & .322 & .734 & .604 & .579 & .569 \\
        \textsc{GCN-Mean} & .772 & \textbf{.616} & \textbf{.594} & .778 & .659 & \textbf{.835} & \textbf{.709} \\
        \bottomrule
    \end{tabular}
\end{small}



% \begin{tabular}{rcccccccccc}
% \toprule
%  & \textsc{LSTM-Bi} & \textsc{LSTM-BiE} & \textsc{DOM-Q-NET}  & \textsc{FreeDOM} & \textsc{FreeDOM-ext} &
%  \textsc{FCN} & \textsc{GAT} & \textsc{LSTM-TD} & \textsc{TE} & \textsc{PinSage} \\
%  \midrule
%  BuyButton & .720 & .773 & .775 & .379 & .840 & .786 & .255 & .714 & .708 & .772 \\
%  Cart & .570 & .596 &.576  & .061 & .588 & .530 & .043 & .512 & .468 & .616 \\
%  Picture & .466 & .503 & .400 & .020 & .343 & .320 & .148 & .424 & .322 & .594 \\
%  Name & .693 & .724 & .700 & .645 & .835 & .702 & .654 & .696 & .734 & .778 \\
%  Price & .483 & .546 & .504 & .245 & .728 & .575 & .109 & .523 & .604 & .659 \\
%  SubjectNode & .656 & .702 & .462 & .334 & .479 & .433 & .018 & .584 & .579 & .835 \\
%  Avg. & .598 & .641 & .569 & .281 & .635 & .558 & .204 & .575 & .569 & .709 \\
%  \bottomrule
% \end{tabular}


% Raw data
% \textsc{LSTM-Bi} & .7198 & .5698 & .4661 & .6933 & .483 & .6558 & .5979666666666666 \\
% \textsc{LSTM-BiE} & .7726 & .5959 & .5031 & .7243 & .5458 & .7015 & .6405333333333333 \\
% \textsc{DOM-Q-NET} & .7753 &.5756 & .3999 & .6995 & .504 & .4624 & .56945 \\
% \textsc{FreeDOM} & .3792 &.0608 & .02 & .6451 & .2446 & .334 & .2806166666666667 \\
% \textsc{FreeDOM-ext} & .8397 & .5875 & .3434 & .8351 & .728 & .4791 & .6354666666666667 \\
% \textsc{FCN} & .786 & .5298 & .3199 & .7015 & .575 & .4332 & .5575666666666667 \\
% \textsc{GAT} & .2548 & .0426 & .1479 & .6536 & .1093 & .0179 & .20435 \\
% \textsc{LSTM-TD} & .7135 & .5119 & .4239 & .6959 & .5228 & .584 & .5753333333333334 \\
% \textsc{TE} & .7083 & .4679 & .3215 & .7343 & .6038 & .5792 & .5691666666666667 \\
% \textsc{PinSage} & .772 & .6156 & .5939 & .7779 & .6587 & .835 & .7088500000000001\\


==> tables/prediction-text-table.tex <==
\begin{small}
    \centering
    \begin{tabular}{rccccccc}
        \toprule
        & buy button & cart button & product image & name & price & subject node & avg. \\
        \midrule
        \textsc{LSTM-BU-T} & .897 & .645 & .423 & .733 & .563 & .552 & .636 \\
        \textsc{GCN-GRU-T} & .837 & .620 & .373 & .791 & .607 & .514 & .624 \\
        \textsc{FreeDOM} & .379 & .061 & .020 & .645 & .245 & .334 & .281 \\
        \textsc{FreeDOM-ext} & .840 & .588 & .343 & \textbf{.835} & \textbf{.728} & .479 & .635 \\
        \textsc{FCN-T} & .862 & .615 & .277 & \textbf{.835} & .616 & .435 & .607 \\
        \textsc{LSTM-TD-T} & .856 & .559 & .438 & .771 & .586 & .390 & .600 \\
        \textsc{TE-T} & .814 & .495 & .369 & .787 & .611 & .619 & .616 \\
        \textsc{GCN-Mean-T} & \textbf{.911} & \textbf{.671} & \textbf{.497} & .811 & .653 & \textbf{.855} & \textbf{.733}\\
        \bottomrule
    \end{tabular}
\end{small}

% RAW DATA
% method,addtocart,average,cart,mainpicture,name,price,subjectnode
% BottomUP-T,.897,.636,.645,.423,.733,.563,.552
% DOMQNET-T,.837,.624,.620,.373,.791,.607,.514
% FreeDOM,.379,.281,.061,.020,.645,.245,.334
% FreeDOM-ext,.840,.635,.588,.343,.835,.728,.479
% FullyConnected-T,.862,.607,.615,.277,.835,.616,.435
% TopDown-T,.856,.600,.559,.438,.771,.586,.390
% TransformerEncoder-T,.814,.616,.495,.369,.787,.611,.619
% TwoLayerGCN-T,.911,.733,.671,.497,.811,.653,.855


==> tikz-figures/big_dom_tree.tex <==
\begin{scope}[scale=1]
    \begin{scope}[xshift=-6.35cm,yshift=2.55cm] 
\node[fillednode]  (body) {body};
\node (empty1) [fillednode,below left=of body]{$\quad$};
\node (empty2) [fillednode,below right=of body]{$\quad$};
\node (cart) [fillednode,below left =of empty2, xshift = 0.5cm]{Cart};
\node (empty3) [fillednode,below right =of empty2, xshift = -0.5cm]{$\quad$};
\node (buy) [fillednode,below  =of empty3, yshift=0.2cm]{Buy};
\node (img) [fillednode, below =of empty1, yshift=8pt]{Img};
\node (empty4) [fillednode, below left = of buy , xshift = 0.5cm, yshift=0.2cm]{$\quad$};
\node (empty5) [fillednode, below right= of buy , xshift = -0.5cm, yshift=0.2cm]{$\quad$};
\draw[very thick, black!60] (body) -- (empty1);
\draw[very thick, black!60] (body) -- (empty2);
\draw[dotted, very thick, black!60] (empty1) -- (img);
\draw[dotted, very thick, black!60] (empty2) -- (cart);
\draw[dotted, very thick, black!60] (empty2) -- (empty3);
\draw[very thick, black!60] (empty3) -- (buy);
\draw[very thick, black!60] (buy) -- (empty4);
\draw[very thick, black!60] (buy) -- (empty5);

%\node [draw=red, fit= (buy) (empty4) (empty5) (empty3), inner sep=0.05cm, rounded corners] {};

\begin{pgfonlayer}{background}
% Area around buy button
 % \draw[rounded corners = 9pt, thick, fill=C7!80!black, opacity=0.2] ([xshift = -5pt,yshift = 5pt]empty4.north west)  .. controls ([xshift = -15pt]buy.west) ..  ([xshift = -10pt]empty3.west)  .. controls ([yshift = 5pt, xshift = -5pt]empty3.north west) .. ([yshift = 10pt]empty3.north)  .. controls ([yshift = 5pt, xshift = 5pt]empty3.north east) .. ([xshift = 10pt]empty3.east) .. controls ([xshift = 5pt,yshift=5pt]empty5.north east) ..([xshift=10pt]empty5.east)  .. controls ([xshift=5pt, yshift =-5pt]empty5.south east) .. ([yshift=-10pt]empty5.south) .. controls  ([xshift = 5pt,yshift = -5pt]empty4.south east) ..  ([yshift = -10pt]empty4.south) .. controls ([xshift = -5pt,yshift = -5pt]empty4.south west) .. ([xshift = -10pt]empty4.west) -- cycle;
  \draw[rounded corners = 9pt, thick, fill=C7!80!black, opacity=0.2] ([xshift = -5pt,yshift = 5pt]empty4.north west)  .. controls ([xshift = -10pt]buy.west) and ([yshift = 10pt, xshift = -10pt]buy.north)  ..  ([xshift = -10pt]empty3.west)  .. controls ([yshift = 5pt, xshift = -5pt]empty3.north west) .. ([yshift = 10pt]empty3.north)  .. controls ([yshift = 5pt, xshift = 5pt]empty3.north east) .. ([xshift = 10pt]empty3.east) .. controls ([yshift = 10pt, xshift = 16pt]buy.north)  .. ([xshift = 15pt]buy.east) .. controls ([xshift = 5pt,yshift=5pt]empty5.north east) ..([xshift=10pt]empty5.east)  .. controls ([xshift=5pt, yshift =-5pt]empty5.south east) .. ([yshift=-10pt]empty5.south) .. controls ([xshift = -5pt,yshift=-5pt]empty5.south west) .. ([xshift = -10pt]empty5.west) .. controls  ([yshift=-28pt]buy.south) .. ([xshift = 10pt]empty4.east) .. controls ([xshift = 5pt,yshift = -5pt]empty4.south east) ..  ([yshift = -10pt]empty4.south) .. controls ([xshift = -5pt,yshift = -5pt]empty4.south west) .. ([xshift = -10pt]empty4.west) -- cycle;

      % Additional, larger area around all nodes
  \draw[rounded corners = 9pt, thick, fill=C8!80!black, opacity=0.2]
  ([xshift = -12pt]empty4.west) .. controls ([xshift = -20pt]buy.west) ..
  ([yshift = -10pt]cart.south) .. controls  ([yshift = -10pt]img.south) ..
     ([yshift = -5pt, xshift =-5pt]img.south west) .. controls  ([xshift = -10pt]img.west) ..([ xshift = -10pt]empty1.west) .. controls ([yshift = 5pt, xshift = -5pt]empty1.north west)..
     ([xshift = -10pt]body.west)  .. controls ([yshift = 5pt, xshift = -5pt]body.north west) .. ([yshift = 10pt]body.north) ..  controls ([yshift = 5pt, xshift = 5pt]body.north east) .. ([xshift = 10pt]body.east)  .. controls ([yshift = 5pt, xshift = 5pt]empty2.north east)  .. ([ xshift = 10pt]empty2.east) .. controls  ([yshift = 7pt, xshift = 7pt]empty3.north east) .. ([xshift = 12pt]empty3.east) .. controls ([xshift = 12pt]empty5.east) ..  ([yshift = -7pt, xshift = 7pt]empty5.south east)  .. controls ([yshift = -12pt]empty5.south) and  ([yshift = -12pt]empty4.south)..  ([yshift = -7pt, xshift = -7pt]empty4.south west)
     -- cycle;
\end{pgfonlayer}

\end{scope}
\end{scope}


==> tikz-figures/classification.tex <==

\node (title) at (0,0) [above, yshift=2.75cm, xshift = 3.3cm] {\Large\textbf{Classification: Which Class does this Element belong to?}};

\begin{scope}[scale=0.65,xshift=2.75cm,yshift=1cm]
    \begin{scope}[ xshift=1cm, yshift=1cm] 


    %\node[yshift=0.25cm] (features) {Node features ($\bx$)};
    %\node[yshift=-0.25cm] (context) {DOM tree context};
    %\coordinate (input); 
    \node[draw,very thick,C6, fill=C6!50, trapezium, trapezium angle=75, shape border rotate=270, minimum
        width=0.64cm, minimum height=0.32cm, label={[yshift=-0.1cm, text = black!72]below:Embedder}] (embedder) {};
%     text = black!72,
    % \node[draw, rectangle, minimum height=1cm, right=1cm of embedder] (classifier) {classifier};
    \node[draw, very thick, C4, fill=C4!50, trapezium, trapezium angle=75, shape border rotate=270, minimum width=0.64cm, minimum height=0.32cm,  label={[yshift=-0.1cm, text = black!72]below:Classifier}, right=1cm of embedder] (classifier) {};
    % \node[trapezium, trapezium angle=85,rotate=90, minimum width=4cm, draw, right=1cm of embedder] (classifier) {classifier};
    \node[right=1cm of classifier] (output){$\quad$};
    
    \draw[-latex, black!60,  thick] ([xshift =0.1cm]embedder.east) to coordinate[midway] (z) ([xshift =-0.1cm]classifier.west);

    %      \draw[-latex, black!60,  thick] ([xshift =0.1cm]buy2.east) to ([xshift =-0.1cm]embedder.west);
    \draw[-latex, black!60,  thick] ([xshift =0.1cm]classifier.east) to (output);


     \node (buy2) [fillednode2, left  =of embedder, xshift = -0.5cm]{Buy};
     \node (empty32) [fillednode2, above =of buy2, yshift =-0.75cm]{$\quad$};
    \node (empty42) [fillednode2, below left = of buy2 , xshift = 0.7cm, yshift =0.75cm]{$\quad$};
    \node (empty52) [fillednode2, below right= of buy2 , xshift = -0.7cm, yshift =0.75cm]{$\quad$};
     \draw[very thick, black!60] (empty32) -- (buy2);
     \draw[very thick, black!60] (buy2) -- (empty42);
     \draw[very thick, black!60] (buy2) -- (empty52);
     \draw[-latex, black!60,  thick] ([xshift =0.1cm]buy2.east) to ([xshift =-0.1cm]embedder.west);
    \draw[very thick,-latex, C7, dotted] ([yshift = 4pt, xshift= 6.5pt]empty3.north east) to[bend left=45] ([xshift=-5pt,yshift=5pt]buy2.west);
    
\end{scope}


\begin{scope}[xshift=5.85cm,yshift=0.5cm] % Adjust the xshift value as needed to place the histogram
\begin{axis}[
    ybar, % Bar plot
    width = 0.27\linewidth,
    height = 0.18\linewidth,
    bar width=10pt, % Width of the bars
    symbolic x coords={Cart, Buy, Img, Price, Subject Node, Unlabeled}, % Categories
    xtick=data, % Place ticks at data points
    x tick label style={rotate=45, anchor=east, text=black!72},
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides
    xtick style={draw=none}, % No tick lines for x-axis
    ytick style={draw=none,}, % No tick lines for y-axis
    y tick label style={text=black!72},
    ymax =1.1,
    ymin=-0.1,
    % Customize axis lines to be thicker
    x axis line style={black!60,-, line width=0.8pt}, % Make x-axis line thicker
    y axis line style={black!60, -, line width=0.8pt}, % Make y-axis line thicker
]

\addplot[fill=C2!60, draw=C2, thick] coordinates {
    (Cart, 0.02) 
    (Buy, 0.9) 
    (Img, 0.02) 
    (Price, 0.02) 
    (Subject Node, 0.02) 
    (Unlabeled, 0.02)
};
\end{axis}

\end{scope}


\end{scope}


==> tikz-figures/hard_labels_confidence_gcn_aggregated.tex <==
\tikzstyle{s0}=[very thick,densely dashed, C6]
\tikzstyle{s1}=[very thick,densely dashed, C7]
\tikzstyle{s2}=[very thick,densely dashed, C8]
\tikzstyle{s3}=[very thick,densely dashed, C9]
\tikzstyle{s4}=[very thick,densely dashed, C0]
\tikzstyle{s5}=[very thick,densely dashed, C1]
\tikzstyle{s6}=[very thick, C6]
\tikzstyle{s7}=[very thick, C7]
\tikzstyle{s8}=[very thick, C8]
\tikzstyle{s9}=[very thick, C9]
\tikzstyle{s10}=[very thick, C0]
\tikzstyle{s11}=[very thick, C1]


% add to cart
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_with_aug/run-version_6_confidence_gap_addtocart-tag-confidence_gap.csv}\augall
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_with_aug/run-version_6_confidence_gap_cart-tag-confidence_gap.csv}\augcart
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_with_aug/run-version_6_confidence_gap_mainpicture-tag-confidence_gap.csv}\augmainpicture
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_with_aug/run-version_6_confidence_gap_name-tag-confidence_gap.csv}\augname
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_with_aug/run-version_6_confidence_gap_price-tag-confidence_gap.csv}\augprice
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_with_aug/run-version_6_confidence_gap_subjectnode_prod-tag-confidence_gap.csv}\augsubjectnode

\pgfplotstablecreatecol[
  copy column from table={\augcart}{[index] 2},
  ]{Value2}{\augall}
  \pgfplotstablecreatecol[
  copy column from table={\augmainpicture}{[index] 2},
  ]{Value3}{\augall}
\pgfplotstablecreatecol[
  copy column from table={\augname}{[index] 2},
  ]{Value4}{\augall}
 \pgfplotstablecreatecol[
  copy column from table={\augprice}{[index] 2},
  ]{Value5}{\augall}
 \pgfplotstablecreatecol[
  copy column from table={\augsubjectnode}{[index] 2},
  ]{Value6}{\augall}



\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_no_aug/run-version_15_confidence_gap_addtocart-tag-confidence_gap.csv}\noaugall
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_no_aug/run-version_15_confidence_gap_cart-tag-confidence_gap.csv}\noaugcart
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_no_aug/run-version_15_confidence_gap_mainpicture-tag-confidence_gap.csv}\noaugmainpicture
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_no_aug/run-version_15_confidence_gap_name-tag-confidence_gap.csv}\noaugname
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_no_aug/run-version_15_confidence_gap_price-tag-confidence_gap.csv}\noaugprice
\pgfplotstableread[col sep=comma]{figure-data/hard-labels/confidence_gap_no_aug/run-version_15_confidence_gap_subjectnode_prod-tag-confidence_gap.csv}\noaugsubjectnode



\pgfplotstablecreatecol[
  copy column from table={\noaugcart}{[index] 2},
  ]{Value2}{\noaugall}
  \pgfplotstablecreatecol[
  copy column from table={\noaugmainpicture}{[index] 2},
  ]{Value3}{\noaugall}
  \pgfplotstablecreatecol[
  copy column from table={\noaugname}{[index] 2},
  ]{Value4}{\noaugall}
   \pgfplotstablecreatecol[
  copy column from table={\noaugprice}{[index] 2},
  ]{Value5}{\noaugall}
   \pgfplotstablecreatecol[
  copy column from table={\noaugsubjectnode}{[index] 2},
  ]{Value6}{\noaugall}
  

\begin{tikzpicture}
\begin{axis}[
        legend style={at={(0.5, -0.3)},
            anchor= north, legend columns=3,
            nodes={scale=0.65}
        },
        width  = \columnwidth,
        height = 6cm,
        scaled y ticks = false,
        ylabel = {Avg. Confidence Gap},
        xlabel = {\# of batches},
        ymajorgrids = true,]
\addplot[s6] table[x index=1,y expr= (\thisrow{Value}+\thisrow{Value2}+\thisrow{Value3}+\thisrow{Value4}+\thisrow{Value5}+\thisrow{Value6})/6 ]{\augall};
\addlegendentry{hard-labels};
\addplot[s9] table[x index=1,y expr= (\thisrow{Value}+\thisrow{Value2}+\thisrow{Value3}+\thisrow{Value4}+\thisrow{Value5}+\thisrow{Value6})/6 ]{\noaugall};
\addlegendentry{no-hard-labels};

\end{axis}
\end{tikzpicture}

==> tikz-figures/increasing-data.tex <==
\tikzstyle{s0}=[very thick, mark=*, C6]
\tikzstyle{s1}=[very thick, mark=*, C7]
\tikzstyle{s2}=[very thick, mark=*, C8]
\tikzstyle{s3}=[very thick, mark=*, C9]
\tikzstyle{s4}=[very thick, mark=*, C0]
\tikzstyle{s5}=[very thick, mark=*, C1]
\tikzstyle{s6}=[very thick, mark=*, C2]
\tikzstyle{s7}=[very thick, mark=*, C3]
\tikzstyle{s8}=[very thick, mark=*, C4]
\tikzstyle{s9}=[very thick, mark=*, C5]


\pgfplotstableread[col sep=comma]{figure-data/increasing_data_experiments.csv}\data
\begin{tikzpicture}[outer sep = 0pt]
    \begin{axis}[
        legend style={at={(0.5, -0.4)},
            anchor= north, legend columns=4,
            nodes={scale=0.8}
        },
        legend cell align=left,
        ylabel={\#participants},
        % nodes near coords,
        % nodes near coords align={vertical},
        width  = 0.85\columnwidth,
        height = 5cm,
        ymajorgrids = true,
        ylabel = {Predictive accuracy},
        xlabel = {Training dataset size},
        scaled y ticks = false,
        xmode=log,
        xmin = 120,
        xmax = 11000,
        log basis x={2},
        ymin=0.19,
        ymax=0.81,
        yticklabel style={/pgf/number format/skip 0.=true},
    ]

    \addplot[s0] table[x index=0,y=TwoLayerGCN] {\data};
    \addlegendentry{GCN-Mean};
    \addplot[s1] table[x index=0,y=BidirectionalWithEmbeddings] {\data};
    \addlegendentry{LSTM-BiE};
    \addplot[s2] table[x index=0,y=FreeDOM] {\data};
    \addlegendentry{FreeDOM-ext};
    \addplot[s4] table[x index=0,y=TransformerEncoder] {\data};
    \addlegendentry{TE};
    \addplot[s5] table[x index=0,y=DOMQNET] {\data};
    \addlegendentry{GCN-GRU};
    \addplot[s6] table[x index=0,y=FullyConnected] {\data};
    \addlegendentry{FCN};
    \addplot[s7] table[x index=0,y=TopDown] {\data};
    \addlegendentry{LSTM-TD};
    \addplot[s8] table[x index=0,y=Bidirectional] {\data};
    \addlegendentry{LSTM-Bi};
    \end{axis}%
\end{tikzpicture}%



%     \addplot[f0] table[x=class, y=TwoLayerGCN] {\datatuned};
%     \addplot[f1] table[x=class, y=BidirectionalLSTMWithEmbeddings] {\datatuned};
%     \addplot[f2] table[x=class, y=FreeDOM-ext] {\datatuned};
%     \addplot[f3] table[x=class, y=BottomUpLSTM] {\datatuned};
%     \addplot[f4] table[x=class, y=TransformerEncoder] {\datatuned};
%     \addplot[f5] table[x=class, y=DOMQNET] {\datatuned};
%     \addplot[f6] table[x=class, y=FullyConnected] {\datatuned};
%     \addplot[f7] table[x=class, y=TopDownLSTM] {\datatuned};
%     \addplot[f8] table[x=class, y=BidirectionalLSTM] {\datatuned};
%     \addplot[f9] table[x=class, y=FreeDOM] {\datatuned};

==> tikz-figures/nomination.tex <==
\begin{scope}[yshift=2cm, xshift = 1cm]
 \node (title) at (0,0) [above, yshift=-2.8cm, xshift = 2.7cm] {\Large\textbf{Nomination: Which Element on the Page is the Buy Button?}};
\begin{scope}[xshift =-1cm]
\begin{scope}[yshift=0cm]


\begin{scope}[xshift = -0.8cm]
  \input{tikz-figures/unsorted_ranking}  
\end{scope}




\end{scope}




 %     \node[draw,very thick,C6, fill=C6!50, trapezium, trapezium angle=75, shape border rotate=270, minimumwidth=0.8cm, minimum height=0.4cm, label={[yshift=-0.1cm]below:Embedder}] (embedder) {};
\end{scope}

    \node(A) at (1,-2.989) {$\quad$};
  \node(B) at (1.1,-4.8945) {$\quad$};
  \node(C) at (1,-6.8) {$\quad$};
  \node(D) at (3.3,-4.8945) {$\quad$};



 \draw [ thick,black!60, decorate,decoration={brace,amplitude=4pt},xshift=0.5cm,yshift=0pt]
      (A) -- (C) node [midway,right,xshift=.1cm] {$\quad$};

      \draw [thick, -latex, black!60, text = black!72] (B.east) -- (D) node[midway,below] {RANK};
 % \node(Compare) at (5,-4.6) {Rank};

 % \draw[-latex] (A) to (Compare);
  %\draw[-latex] (B) to (Compare);
  %\draw[-latex] (C) to (Compare);


\begin{scope}[xshift=4cm]
    \input{tikz-figures/sorted_ranking}
\end{scope}



  
   \node(Final) at (7.5,-4.6) {$\quad$};
       
       
     %  \begin{scope}[shift={(Final)}]
       % Now the coordinate (0,0) is at the 'Final' node position
      % \node (empty54) [fillednode3] at (0,0) {$\quad$}; % Positioned at 'Final'
      % \node (empty55) [fillednode3, below left=of empty54, yshift=0.7cm, xshift=1cm] {$\quad$};
      % \node (empty56) [fillednode3, below right=of empty54, yshift=0.7cm, xshift=-1cm] {$\quad$};
       %\draw[very thick, black!60] (empty54) -- (empty55);
       %\draw[very thick, black!60] (empty54) -- (empty56);
   %\end{scope}


  %\draw[-latex] (Compare) to (Final);

   % \node (finallabel) [above = of Final, yshift= -0.7cm] {Nominate Buy Button};
    
\end{scope}






==> tikz-figures/sorted_ranking.tex <==
\begin{scope}[scale =0.75,xshift=1cm,yshift=-5.25cm] % Adjust the xshift value as needed to place the histogram
\begin{axis}[
    ybar, % Bar plot
    width = 0.21\linewidth,
    height = 0.14\linewidth,
    %title = \textbf{Nomination:} Which Element on the Page is the Cart?,
    bar width=7pt, % Width of the bars
    symbolic x coords={Cart, Buy, Img, Price, Subject Node, Unlabeled}, % Categories
    xtick=data, % Place ticks at data points
    xticklabels={},
    yticklabels={},
   % x tick label={}, % Hide x-axis tick label style={rotate=45, anchor=east},
    %axis lines*=left, % Only show the left axis line
    %axis x line*=bottom, % Only show the bottom axis line
    %axis line style={-}, % Remove arrow tips from axis lines
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides
    xtick style={draw=none}, % No tick lines for x-axis
    ytick style={draw=none}, % No tick lines for y-axis
    x axis line style={black!60,-, line width=0.8pt}, % Make x-axis line thicker
    y axis line style={black!60, -, line width=0.8pt},
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides%ymajorgrids, % Enable horizontal grid lines
    ymax =1.1,
    ymin=-0.1,
    %grid style={dashed,gray!30}, % Customize grid style
]

% Sample data with specified border color
\addplot[fill=C2!60, draw=C2, thick] coordinates {
    (Cart, 0.01) 
    (Buy, 0.99) 
    (Img, 0.01) 
    (Price, 0.01) 
    (Subject Node, 0.01) 
    (Unlabeled, 0.01)
};
\end{axis}
\end{scope}
\begin{scope}[scale =0.75,xshift=1cm,yshift=-6.5cm] % Adjust the xshift value as needed to place the histogram
\begin{axis}[
    ybar, % Bar plot
    width = 0.21\linewidth,
    height = 0.14\linewidth,
    %title = \textbf{Nomination:} Which Element on the Page is the Cart?,
    bar width=7pt, % Width of the bars
    symbolic x coords={Cart, Buy, Img, Price, Subject Node, Unlabeled}, % Categories
    xtick=data, % Place ticks at data points
    xticklabels={},
    yticklabels={},
   % x tick label={}, % Hide x-axis tick label style={rotate=45, anchor=east},
    %axis lines*=left, % Only show the left axis line
    %axis x line*=bottom, % Only show the bottom axis line
    %axis line style={-}, % Remove arrow tips from axis lines
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides
    xtick style={draw=none}, % No tick lines for x-axis
    ytick style={draw=none}, % No tick lines for y-axis
    x axis line style={black!60,-, line width=0.8pt}, % Make x-axis line thicker
    y axis line style={black!60, -, line width=0.8pt},
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides%ymajorgrids, % Enable horizontal grid lines
    ymax =1.1,
    ymin=-0.1,
    %grid style={dashed,gray!30}, % Customize grid style
]

% Sample data with specified border color
\addplot[fill=C2!60, draw=C2, thick] coordinates {
    (Cart, 0.0375) 
    (Buy, 0.75) 
    (Img, 0.0375) 
    (Price, 0.0375) 
    (Subject Node, 0.0375) 
    (Unlabeled, 0.2)
};
\end{axis}
\end{scope}

\node[very thick, black!60] at (1.5,-5.25) {$\vdots$};
\begin{scope}[scale =0.75,xshift=1cm,yshift=-8.75cm] % Adjust the xshift value as needed to place the histogram
\begin{axis}[
    ybar, % Bar plot
    width = 0.21\linewidth,
    height = 0.14\linewidth,
    %title = \textbf{Nomination:} Which Element on the Page is the Cart?,
    bar width=7pt, % Width of the bars
    symbolic x coords={Cart, Buy, Img, Price, Subject Node, Unlabeled}, % Categories
    xtick=data, % Place ticks at data points
    xticklabels={},
    yticklabels={},
   % x tick label={}, % Hide x-axis tick label style={rotate=45, anchor=east},
    %axis lines*=left, % Only show the left axis line
    %axis x line*=bottom, % Only show the bottom axis line
    %axis line style={-}, % Remove arrow tips from axis lines
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides
    xtick style={draw=none}, % No tick lines for x-axis
    ytick style={draw=none}, % No tick lines for y-axis
    x axis line style={black!60,-, line width=0.8pt}, % Make x-axis line thicker
    y axis line style={black!60, -, line width=0.8pt},
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides%ymajorgrids, % Enable horizontal grid lines
    ymax =1.1,
    ymin=-0.1,
    %grid style={dashed,gray!30}, % Customize grid style
]

% Sample data with specified border color
\addplot[fill=C2!60, draw=C2, thick] coordinates {
   (Cart, 0.01) 
    (Buy, 0.01) 
    (Img, 0.01) 
    (Price, 0.01) 
    (Subject Node, 0.01) 
    (Unlabeled, 0.95)
};
\end{axis}
\end{scope}


  \begin{scope}[yshift=-3.475cm] 

\node (empty541) [fillednode3]{$B$};
  \node (empty540) [fillednode3, above=of empty541, yshift=-0.85cm]{$\quad$};
\node (empty552) [fillednode3, below left=of empty541, yshift=0.85cm, xshift = 1cm]{$\quad$};
\node (empty563) [fillednode3, below right=of empty541, yshift=0.85cm, , xshift = -1cm]{$\quad$};
\draw[very thick, black!60] (empty540) -- (empty541);
\draw[very thick, black!60] (empty541) -- (empty552);
\draw[very thick, black!60] (empty541) -- (empty563);
\end{scope}

\node [draw, thick, C3, dotted, very thick, rectangle, minimum width=3cm, xshift = 1.1cm, minimum height=1.1cm, fit=(empty540) (empty552) (empty563), inner sep=0pt] (myRectangle) at (empty541) {};
% Adding a label to the right of the rectangle
\node [black,xshift = -0.7cm,yshift =0.05cm, right=of myRectangle.east, anchor=west, align=left, text = black!72] {Nominate\\Buy Button\\Element};
    \begin{scope}[xshift=0cm,yshift=-4.4cm]
\node (empty5410) [fillednode3]{$\quad$};

\node (empty5522) [fillednode3, below left=of empty5410, yshift=0.85cm, xshift = 0.8cm]{$\quad$};
\node (empty5543) [fillednode3, below =of empty5410, yshift=0.85cm]{$\quad$};
\node (empty5634) [fillednode3, below right=of empty5410, yshift=0.85cm, xshift = -0.8cm]{$\quad$};
\draw[very thick, black!60] (empty5410) -- (empty5522);
\draw[very thick, black!60] (empty5410) -- (empty5634);
\draw[very thick, black!60] (empty5410) -- (empty5543);

\end{scope}




  \begin{scope}[xshift=0cm,yshift=-6.25cm] 
    \node (empty54) [fillednode3]{$\quad$};
\node (empty55) [fillednode3, below left=of empty54, yshift=0.85cm, xshift = 1cm]{$\quad$};
\node (empty56) [fillednode3, below right=of empty54, yshift=0.85cm, , xshift = -1cm]{$\quad$};
\draw[very thick, black!60] (empty54) -- (empty55);
\draw[very thick, black!60] (empty54) -- (empty56);
\end{scope}



% Last small set of nodes



==> tikz-figures/unsorted_ranking.tex <==
\begin{scope}[scale =0.75,xshift=1cm,yshift=-5.25cm] % Adjust the xshift value as needed to place the histogram
\begin{axis}[
    ybar, % Bar plot
    width = 0.21\linewidth,
    height = 0.14\linewidth,
    %title = \textbf{Nomination:} Which Element on the Page is the Cart?,
    bar width=7pt, % Width of the bars
    symbolic x coords={Cart, Buy, Img, Price, Subject Node, Unlabeled}, % Categories
    xtick=data, % Place ticks at data points
    xticklabels={},
    yticklabels={},
   % x tick label={}, % Hide x-axis tick label style={rotate=45, anchor=east},
    %axis lines*=left, % Only show the left axis line
    %axis x line*=bottom, % Only show the bottom axis line
    %axis line style={-}, % Remove arrow tips from axis lines
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides
    xtick style={draw=none}, % No tick lines for x-axis
    ytick style={draw=none}, % No tick lines for y-axis
    x axis line style={black!60,-, line width=0.8pt}, % Make x-axis line thicker
    y axis line style={black!60, -, line width=0.8pt},
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides%ymajorgrids, % Enable horizontal grid lines
    ymax =1.1,
    ymin=-0.1,
    %grid style={dashed,gray!30}, % Customize grid style
]

% Sample data with specified border color
\addplot[fill=C2!60, draw=C2, thick] coordinates {
    (Cart, 0.01) 
    (Buy, 0.01) 
    (Img, 0.01) 
    (Price, 0.01) 
    (Subject Node, 0.01) 
    (Unlabeled, 0.95)
};
\end{axis}
\end{scope}
\begin{scope}[scale =0.75,xshift=1cm,yshift=-6.5cm] % Adjust the xshift value as needed to place the histogram
\begin{axis}[
    ybar, % Bar plot
    width = 0.21\linewidth,
    height = 0.14\linewidth,
    %title = \textbf{Nomination:} Which Element on the Page is the Cart?,
    bar width=7pt, % Width of the bars
    symbolic x coords={Cart, Buy, Img, Price, Subject Node, Unlabeled}, % Categories
    xtick=data, % Place ticks at data points
    xticklabels={},
    yticklabels={},
   % x tick label={}, % Hide x-axis tick label style={rotate=45, anchor=east},
    %axis lines*=left, % Only show the left axis line
    %axis x line*=bottom, % Only show the bottom axis line
    %axis line style={-}, % Remove arrow tips from axis lines
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides
    xtick style={draw=none}, % No tick lines for x-axis
    ytick style={draw=none}, % No tick lines for y-axis
    x axis line style={black!60,-, line width=0.8pt}, % Make x-axis line thicker
    y axis line style={black!60, -, line width=0.8pt},
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides%ymajorgrids, % Enable horizontal grid lines
    ymax =1.1,
    ymin=-0.1,
    %grid style={dashed,gray!30}, % Customize grid style
]

% Sample data with specified border color
\addplot[fill=C2!60, draw=C2, thick] coordinates {
    (Cart, 0.247) 
    (Buy, 0.5) 
    (Img, 0.06325) 
    (Price, 0.06325) 
    (Subject Node, 0.06325) 
    (Unlabeled, 0.06325)
};
\end{axis}
\end{scope}

\node(nominationpoint)[very thick, black!60] at (1.5,-5.25) {$\vdots$};
\begin{scope}[scale =0.75,xshift=1cm,yshift=-8.75cm] % Adjust the xshift value as needed to place the histogram
\begin{axis}[
    ybar, % Bar plot
    width = 0.21\linewidth,
    height = 0.14\linewidth,
    %title = \textbf{Nomination:} Which Element on the Page is the Cart?,
    bar width=7pt, % Width of the bars
    symbolic x coords={Cart, Buy, Img, Price, Subject Node, Unlabeled}, % Categories
    xtick=data, % Place ticks at data points
    xticklabels={},
    yticklabels={},
   % x tick label={}, % Hide x-axis tick label style={rotate=45, anchor=east},
    %axis lines*=left, % Only show the left axis line
    %axis x line*=bottom, % Only show the bottom axis line
    %axis line style={-}, % Remove arrow tips from axis lines
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides
    xtick style={draw=none}, % No tick lines for x-axis
    ytick style={draw=none}, % No tick lines for y-axis
    x axis line style={black!60,-, line width=0.8pt}, % Make x-axis line thicker
    y axis line style={black!60, -, line width=0.8pt},
    enlarge x limits=0.15, % Add some space between the outer bars and the plot's sides%ymajorgrids, % Enable horizontal grid lines
    ymax =1.1,
    ymin=-0.1,
    %grid style={dashed,gray!30}, % Customize grid style
]

% Sample data with specified border color
\addplot[fill=C2!60, draw=C2, thick] coordinates {
    (Cart, 0.0075) 
    (Buy, 0.0075) 
    (Img, 0.21) 
    (Price, 0.76) 
    (Subject Node, 0.0075) 
    (Unlabeled, 0.0075)
};
\end{axis}
\end{scope}


    \begin{scope}[yshift=-3.425cm]
    \node (empty13) [fillednode3]{$\quad$};
\node (img) [fillednode3, below =of empty13, yshift=0.85cm]{$\quad$};
\draw[very thick, black!60] (empty13) -- (img);
\end{scope}


  \begin{scope}[xshift=0cm,yshift=-4.4cm]
    \node (empty54) [fillednode3]{$\quad$};
\node (empty55) [fillednode3, below left=of empty54, yshift=0.85cm, xshift = 1cm]{$\quad$};
\node (empty56) [fillednode3, below right=of empty54, yshift=0.85cm, , xshift = -1cm]{$\quad$};
\draw[very thick, black!60] (empty54) -- (empty55);
\draw[very thick, black!60] (empty54) -- (empty56);
\end{scope}



\draw[very thick,-latex, C7, dotted] ([xshift = -3.0cm,yshift =0.6cm]buy.north) to[bend right=45] ([xshift = -2cm,yshift=-0.3cm]nominationpoint);

% Last small set of nodes
  \begin{scope}[xshift=0cm,yshift=-6.25cm]

\node (empty541) [fillednode3]{$\quad$};
  \node (empty540) [fillednode3, above=of empty541, yshift=-0.85cm]{$\quad$};
\node (empty552) [fillednode3, below left=of empty541, yshift=0.85cm, xshift = 0.8cm]{$\quad$};
\node (empty554) [fillednode3, below =of empty541, yshift=0.85cm]{$\quad$};
\node (empty563) [fillednode3, below right=of empty541, yshift=0.85cm, xshift = -0.8cm]{$\quad$};
\draw[very thick, black!60] (empty540) -- (empty541);
\draw[very thick, black!60] (empty541) -- (empty552);
\draw[very thick, black!60] (empty541) -- (empty563);
\draw[very thick, black!60] (empty541) -- (empty554);
\end{scope}
